Footprints of leptoquarks: from $ R_{K^{(*)}} $ to $ K \to \pi \nu \bar\nu $

Rare $K \to \pi \nu \bar \nu$ decays, being dominated by short distance contributions within the Standard Model (SM), open a window for New Physics (NP) searches at low energies. The $ K \to \pi \nu \bar\nu $ branching ratios are expected to be measured with $ \sim 10\% $ accuracies by NA62/CERN and KOTO/JPARC. The theoretical uncertainties of branching ratios within the SM are well under control. In the $ B $ sector, it is tentative to explain the $ B $-meson anomalies $ R_{D^{(\ast)}} $ and/or $ R_{K^{(\ast)}} $ by effects of physics beyond the SM. Although NP seems to be present in the third fermion generation it might also manifest in the flavor changing neutral current transition $ s \to d $. Together with the anticipated good experimental sensitivities and accurate theoretical predictions for $ K\to \pi \nu \bar \nu $, this motivates studies of correlated effects of NP in rare $ K\to \pi \nu \bar \nu $ and $ B \to K^{(*)} \mu^+ \mu^- $ decays. Here we consider the loop induced effects in $ K \to \pi \nu \bar\nu $ in two leptoquark models designed to address lepton-flavor universality violation in the $ R_{K^{(\ast)}} $ anomalies.

==> full_bib_2.tex <==
\begin{thebibliography}{99}
%\cite{Aaij:2014ora}
\bibitem{Aaij:2014ora} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Test of lepton universality using $B^{+}\rightarrow K^{+}\ell^{+}\ell^{-}$ decays,''
  Phys.\ Rev.\ Lett.\  {\bf 113}, 151601 (2014)
  doi:10.1103/PhysRevLett.113.151601
  [arXiv:1406.6482 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.113.151601;%%
  %501 citations counted in INSPIRE as of 02 Feb 2018


%\cite{1705.05802}
\bibitem{1705.05802} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Test of lepton universality with $B^{0} \rightarrow K^{*0}\ell^{+}\ell^{-}$ decays,''
  JHEP {\bf 1708}, 055 (2017)
  doi:10.1007/JHEP08(2017)055
  [arXiv:1705.05802 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP08(2017)055;%%
  %122 citations counted in INSPIRE as of 02 Feb 2018


%\cite{1205.5442}
\bibitem{1205.5442} 
  J.~P.~Lees {\it et al.} [BaBar Collaboration],
  %``Evidence for an excess of $\bar{B} \to D^{(*)} \tau^-\bar{\nu}_\tau$ decays,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 101802 (2012)
  doi:10.1103/PhysRevLett.109.101802
  [arXiv:1205.5442 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.109.101802;%%
  %484 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Lees:2013uzd}
\bibitem{Lees:2013uzd} 
  J.~P.~Lees {\it et al.} [BaBar Collaboration],
  %``Measurement of an Excess of $\bar{B} \to D^{(*)}\tau^- \bar{\nu}_\tau$ Decays and Implications for Charged Higgs Bosons,''
  Phys.\ Rev.\ D {\bf 88}, no. 7, 072012 (2013)
  doi:10.1103/PhysRevD.88.072012
  [arXiv:1303.0571 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.88.072012;%%
  %310 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2015yra}
\bibitem{Aaij:2015yra} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Measurement of the ratio of branching fractions $\mathcal{B}(\bar{B}^0 \to D^{*+}\tau^{-}\bar{\nu}_{\tau})/\mathcal{B}(\bar{B}^0 \to D^{*+}\mu^{-}\bar{\nu}_{\mu})$,''
  Phys.\ Rev.\ Lett.\  {\bf 115}, no. 11, 111803 (2015)
  Erratum: [Phys.\ Rev.\ Lett.\  {\bf 115}, no. 15, 159901 (2015)]
  doi:10.1103/PhysRevLett.115.159901, 10.1103/PhysRevLett.115.111803
  [arXiv:1506.08614 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.115.159901, 10.1103/PhysRevLett.115.111803;%%
  %335 citations counted in INSPIRE as of 02 Feb 2018


%\cite{1507.03233}
\bibitem{1507.03233} 
  M.~Huschle {\it et al.} [Belle Collaboration],
  %``Measurement of the branching ratio of $\bar{B} \to D^{(\ast)} \tau^- \bar{\nu}_\tau$ relative to $\bar{B} \to D^{(\ast)} \ell^- \bar{\nu}_\ell$ decays with hadronic tagging at Belle,''
  Phys.\ Rev.\ D {\bf 92}, no. 7, 072014 (2015)
  doi:10.1103/PhysRevD.92.072014
  [arXiv:1507.03233 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.92.072014;%%
  %276 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hirose:2016wfn}
\bibitem{Hirose:2016wfn} 
  S.~Hirose {\it et al.} [Belle Collaboration],
  %``Measurement of the $\tau$ lepton polarization and $R(D^*)$ in the decay $\bar{B} \to D^* \tau^- \bar{\nu}_\tau$,''
  Phys.\ Rev.\ Lett.\  {\bf 118}, no. 21, 211801 (2017)
  doi:10.1103/PhysRevLett.118.211801
  [arXiv:1612.00529 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.118.211801;%%
  %84 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Sato:2016svk}
\bibitem{Sato:2016svk} 
  Y.~Sato {\it et al.} [Belle Collaboration],
  %``Measurement of the branching ratio of $\bar{B}^0 \rightarrow D^{*+} \tau^- \bar{\nu}_{\tau}$ relative to $\bar{B}^0 \rightarrow D^{*+} \ell^- \bar{\nu}_{\ell}$ decays with a semileptonic tagging method,''
  Phys.\ Rev.\ D {\bf 94}, no. 7, 072007 (2016)
  doi:10.1103/PhysRevD.94.072007
  [arXiv:1607.07923 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.94.072007;%%
  %83 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2017tyk}
\bibitem{Aaij:2017tyk} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Measurement of the ratio of branching fractions $\mathcal{B}(B_c^+\,\to\,J/\psi\tau^+\nu_\tau)$/$\mathcal{B}(B_c^+\,\to\,J/\psi\mu^+\nu_\mu)$,''
  arXiv:1711.05623 [hep-ex].
  %%CITATION = ARXIV:1711.05623;%%
  %20 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2014pli}
\bibitem{Aaij:2014pli} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Differential branching fractions and isospin asymmetries of $B \to K^{(*)} \mu^+ \mu^-$ decays,''
  JHEP {\bf 1406}, 133 (2014)
  doi:10.1007/JHEP06(2014)133
  [arXiv:1403.8044 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP06(2014)133;%%
  %187 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2016flj}
\bibitem{Aaij:2016flj} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Measurements of the S-wave fraction in $B^{0}\rightarrow K^{+}\pi^{-}\mu^{+}\mu^{-}$ decays and the $B^{0}\rightarrow K^{\ast}(892)^{0}\mu^{+}\mu^{-}$ differential branching fraction,''
  JHEP {\bf 1611}, 047 (2016)
  Erratum: [JHEP {\bf 1704}, 142 (2017)]
  doi:10.1007/JHEP11(2016)047, 10.1007/JHEP04(2017)142
  [arXiv:1606.04731 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP11(2016)047, 10.1007/JHEP04(2017)142;%%
  %49 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2015esa}
\bibitem{Aaij:2015esa} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Angular analysis and differential branching fraction of the decay $B^0_s\to\phi\mu^+\mu^-$,''
  JHEP {\bf 1509}, 179 (2015)
  doi:10.1007/JHEP09(2015)179
  [arXiv:1506.08777 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP09(2015)179;%%
  %142 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aaij:2015oid}
\bibitem{Aaij:2015oid} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Angular analysis of the $B^{0} \to K^{*0} \mu^{+} \mu^{-}$ decay using 3 fb$^{-1}$ of integrated luminosity,''
  JHEP {\bf 1602}, 104 (2016)
  doi:10.1007/JHEP02(2016)104
  [arXiv:1512.04442 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP02(2016)104;%%
  %255 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Abdesselam:2016llu}
\bibitem{Abdesselam:2016llu} 
  A.~Abdesselam {\it et al.} [Belle Collaboration],
  %``Angular analysis of $B^0 \to K^\ast(892)^0 \ell^+ \ell^-$,''
  arXiv:1604.04042 [hep-ex].
  %%CITATION = ARXIV:1604.04042;%%
  %92 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Wehle:2016yoi}
\bibitem{Wehle:2016yoi} 
  S.~Wehle {\it et al.} [Belle Collaboration],
  %``Lepton-Flavor-Dependent Angular Analysis of $B\to K^\ast \ell^+\ell^-$,''
  Phys.\ Rev.\ Lett.\  {\bf 118}, no. 11, 111801 (2017)
  doi:10.1103/PhysRevLett.118.111801
  [arXiv:1612.05014 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.118.111801;%%
  %80 citations counted in INSPIRE as of 02 Feb 2018


%\cite{ATLAS:2017dlm}
\bibitem{ATLAS:2017dlm} 
  The ATLAS collaboration [ATLAS Collaboration],
  %``Angular analysis of $B^0_d \to K^{*}\mu^+\mu^-$ decays in $pp$ collisions at $\sqrt{s}= 8$ TeV with the ATLAS detector,''
  ATLAS-CONF-2017-023.
  %%CITATION = ATLAS-CONF-2017-023;%%
  %39 citations counted in INSPIRE as of 02 Feb 2018


%\cite{CMS:2017ivg}
\bibitem{CMS:2017ivg} 
  CMS Collaboration [CMS Collaboration],
  %``Measurement of the $P_1$ and $P_5'$ angular parameters of the decay $\mathrm{B}^0 \to \mathrm{K}^{*0} \mu^+ \mu^-$ in proton-proton collisions at $\sqrt{s}=8~\mathrm{TeV}$,''
  CMS-PAS-BPH-15-008.
  %%CITATION = CMS-PAS-BPH-15-008;%%
  %35 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Bordone:2017lsy}
\bibitem{Bordone:2017lsy} 
  M.~Bordone, D.~Buttazzo, G.~Isidori and J.~Monnard,
  %``Probing Lepton Flavour Universality with $K \to \pi \nu \bar\nu$ decays,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 9, 618 (2017)
  doi:10.1140/epjc/s10052-017-5202-1
  [arXiv:1705.10729 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-5202-1;%%
  %4 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Bobeth:2016llm}
\bibitem{Bobeth:2016llm} 
  C.~Bobeth, A.~J.~Buras, A.~Celis and M.~Jung,
  %``Patterns of Flavour Violation in Models with Vector-Like Quarks,''
  JHEP {\bf 1704}, 079 (2017)
  doi:10.1007/JHEP04(2017)079
  [arXiv:1609.04783 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP04(2017)079;%%
  %25 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Bobeth:2017ecx}
\bibitem{Bobeth:2017ecx} 
  C.~Bobeth and A.~J.~Buras,
  %``Leptoquarks meet $\varepsilon'/\varepsilon$ and rare Kaon processes,''
  arXiv:1712.01295 [hep-ph].
  %%CITATION = ARXIV:1712.01295;%%
  %4 citations counted in INSPIRE as of 02 Feb 2018


%\cite{DAmbrosio:2017wis}
\bibitem{DAmbrosio:2017wis} 
  G.~D'Ambrosio and A.~M.~Iyer,
  %``Flavour issues in warped custodial models: $B$ anomalies and rare $K$ decays,''
  arXiv:1712.08122 [hep-ph].
  %%CITATION = ARXIV:1712.08122;%%
  %1 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buttazzo:2017ixm}
\bibitem{Buttazzo:2017ixm} 
  D.~Buttazzo, A.~Greljo, G.~Isidori and D.~Marzocca,
  %``B-physics anomalies: a guide to combined explanations,''
  JHEP {\bf 1711}, 044 (2017)
  doi:10.1007/JHEP11(2017)044
  [arXiv:1706.07808 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2017)044;%%
  %28 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Alonso:2015sja}
\bibitem{Alonso:2015sja} 
  R.~Alonso, B.~Grinstein and J.~Martin Camalich,
  %``Lepton universality violation and lepton flavor conservation in $B$-meson decays,''
  JHEP {\bf 1510}, 184 (2015)
  doi:10.1007/JHEP10(2015)184
  [arXiv:1505.05164 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2015)184;%%
  %145 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Dorsner:2017ufx}
\bibitem{Dorsner:2017ufx} 
  I.~Doršner, S.~Fajfer, D.~A.~Faroughy and N.~Košnik,
  %``The role of the $S_3$ GUT leptoquark in flavor universality and collider searches,''
  JHEP {\bf 1710}, 188 (2017)
  doi:10.1007/JHEP10(2017)188
  [arXiv:1706.07779 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2017)188;%%
  %18 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hiller:2014yaa}
\bibitem{Hiller:2014yaa} 
  G.~Hiller and M.~Schmaltz,
  %``$R_K$ and future $b \to s \ell \ell$ physics beyond the standard model opportunities,''
  Phys.\ Rev.\ D {\bf 90}, 054014 (2014)
  doi:10.1103/PhysRevD.90.054014
  [arXiv:1408.1627 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.054014;%%
  %199 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Becirevic:2015asa}
\bibitem{Becirevic:2015asa} 
  D.~Bečirević, S.~Fajfer and N.~Košnik,
  %``Lepton flavor nonuniversality in b→sℓ$^+$ℓ$^-$ processes,''
  Phys.\ Rev.\ D {\bf 92}, no. 1, 014016 (2015)
  doi:10.1103/PhysRevD.92.014016
  [arXiv:1503.09024 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.014016;%%
  %101 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Barbieri:2015yvd}
\bibitem{Barbieri:2015yvd} 
  R.~Barbieri, G.~Isidori, A.~Pattori and F.~Senia,
  %``Anomalies in $B$-decays and $U(2)$ flavour symmetry,''
  Eur.\ Phys.\ J.\ C {\bf 76}, no. 2, 67 (2016)
  doi:10.1140/epjc/s10052-016-3905-3
  [arXiv:1512.01560 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-3905-3;%%
  %95 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Becirevic:2016oho}
\bibitem{Becirevic:2016oho} 
  D.~Bečirević, N.~Košnik, O.~Sumensari and R.~Zukanovich Funchal,
  %``Palatable Leptoquark Scenarios for Lepton Flavor Violation in Exclusive $b\to s\ell_1\ell_2$ modes,''
  JHEP {\bf 1611}, 035 (2016)
  doi:10.1007/JHEP11(2016)035
  [arXiv:1608.07583 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2016)035;%%
  %49 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hiller:2016kry}
\bibitem{Hiller:2016kry} 
  G.~Hiller, D.~Loose and K.~Schönwald,
  %``Leptoquark Flavor Patterns & B Decay Anomalies,''
  JHEP {\bf 1612}, 027 (2016)
  doi:10.1007/JHEP12(2016)027
  [arXiv:1609.08895 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2016)027;%%
  %40 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Chen:2017hir}
\bibitem{Chen:2017hir} 
  C.~H.~Chen, T.~Nomura and H.~Okada,
  %``Excesses of muon $g-2$, $R_{D^{(\ast)}}$, and $R_K$ in a leptoquark model,''
  Phys.\ Lett.\ B {\bf 774}, 456 (2017)
  doi:10.1016/j.physletb.2017.10.005
  [arXiv:1703.03251 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2017.10.005;%%
  %24 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Cheung:2016fjo}
\bibitem{Cheung:2016fjo} 
  K.~Cheung, T.~Nomura and H.~Okada,
  %``Testable radiative neutrino mass model without additional symmetries and explanation for the $b \to s \ell^+ \ell^-$ anomaly,''
  Phys.\ Rev.\ D {\bf 94}, no. 11, 115024 (2016)
  doi:10.1103/PhysRevD.94.115024
  [arXiv:1610.02322 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.115024;%%
  %18 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Cox:2016epl}
\bibitem{Cox:2016epl} 
  P.~Cox, A.~Kusenko, O.~Sumensari and T.~T.~Yanagida,
  %``SU(5) Unification with TeV-scale Leptoquarks,''
  JHEP {\bf 1703}, 035 (2017)
  doi:10.1007/JHEP03(2017)035
  [arXiv:1612.03923 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2017)035;%%
  %15 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Kumar:2016omp}
\bibitem{Kumar:2016omp} 
  G.~Kumar,
  %``Constraints on a scalar leptoquark from the kaon sector,''
  Phys.\ Rev.\ D {\bf 94}, no. 1, 014022 (2016)
  doi:10.1103/PhysRevD.94.014022
  [arXiv:1603.00346 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.014022;%%
  %9 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Crivellin:2017zlb}
\bibitem{Crivellin:2017zlb} 
  A.~Crivellin, D.~Müller and T.~Ota,
  %``Simultaneous explanation of R(D$^{(∗)}$) and b→sμ$^{+}$ μ$^{−}$: the last scalar leptoquarks standing,''
  JHEP {\bf 1709}, 040 (2017)
  doi:10.1007/JHEP09(2017)040
  [arXiv:1703.09226 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2017)040;%%
  %48 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hiller:2017bzc}
\bibitem{Hiller:2017bzc} 
  G.~Hiller and I.~Nisandzic,
  %``$R_K$ and $R_{K^{\ast}}$ beyond the standard model,''
  Phys.\ Rev.\ D {\bf 96}, no. 3, 035003 (2017)
  doi:10.1103/PhysRevD.96.035003
  [arXiv:1704.05444 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.035003;%%
  %64 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Alok:2017sui}
\bibitem{Alok:2017sui} 
  A.~K.~Alok, B.~Bhattacharya, A.~Datta, D.~Kumar, J.~Kumar and D.~London,
  %``New Physics in $b \to s \mu^+ \mu^-$ after the Measurement of $R_{K^*}$,''
  Phys.\ Rev.\ D {\bf 96}, no. 9, 095009 (2017)
  doi:10.1103/PhysRevD.96.095009
  [arXiv:1704.07397 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.095009;%%
  %40 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aloni:2017ixa}
\bibitem{Aloni:2017ixa} 
  D.~Aloni, A.~Dery, C.~Frugiuele and Y.~Nir,
  %``Testing minimal flavor violation in leptoquark models of the $ {R_K}_{{}^{\left(\ast \right)}} $ anomaly,''
  JHEP {\bf 1711}, 109 (2017)
  doi:10.1007/JHEP11(2017)109
  [arXiv:1708.06161 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2017)109;%%
  %5 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Calibbi:2017qbu}
\bibitem{Calibbi:2017qbu} 
  L.~Calibbi, A.~Crivellin and T.~Li,
  %``A model of vector leptoquarks in view of the $B$-physics anomalies,''
  arXiv:1709.00692 [hep-ph].
  %%CITATION = ARXIV:1709.00692;%%
  %17 citations counted in INSPIRE as of 02 Feb 2018


%\cite{DiLuzio:2017vat}
\bibitem{DiLuzio:2017vat} 
  L.~Di Luzio, A.~Greljo and M.~Nardecchia,
  %``Gauge leptoquark as the origin of B-physics anomalies,''
  Phys.\ Rev.\ D {\bf 96}, no. 11, 115011 (2017)
  doi:10.1103/PhysRevD.96.115011
  [arXiv:1708.08450 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.115011;%%
  %15 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Bauer:2015knc}
\bibitem{Bauer:2015knc} 
  M.~Bauer and M.~Neubert,
  %``Minimal Leptoquark Explanation for the R$_{D^{(*)}}$ , R$_K$ , and $(g-2)_g$ Anomalies,''
  Phys.\ Rev.\ Lett.\  {\bf 116}, no. 14, 141802 (2016)
  doi:10.1103/PhysRevLett.116.141802
  [arXiv:1511.01900 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.116.141802;%%
  %138 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Becirevic:2017jtw}
\bibitem{Becirevic:2017jtw} 
  D.~Bečirević and O.~Sumensari,
  %``A leptoquark model to accommodate $R_K^\mathrm{exp} < R_K^\mathrm{SM}$ and $R_{K^\ast}^\mathrm{exp} < R_{K^\ast}^\mathrm{SM}$,''
  JHEP {\bf 1708}, 104 (2017)
  doi:10.1007/JHEP08(2017)104
  [arXiv:1704.05835 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2017)104;%%
  %38 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Cai:2017wry}
\bibitem{Cai:2017wry} 
  Y.~Cai, J.~Gargalionis, M.~A.~Schmidt and R.~R.~Volkas,
  %``Reconsidering the One Leptoquark solution: flavor anomalies and neutrino mass,''
  JHEP {\bf 1710}, 047 (2017)
  doi:10.1007/JHEP10(2017)047
  [arXiv:1704.05849 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2017)047;%%
  %28 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Capdevila:2017bsm}
\bibitem{Capdevila:2017bsm} 
  B.~Capdevila, A.~Crivellin, S.~Descotes-Genon, J.~Matias and J.~Virto,
  %``Patterns of New Physics in $b\to s\ell^+\ell^-$ transitions in the light of recent data,''
  JHEP {\bf 1801}, 093 (2018)
  doi:10.1007/JHEP01(2018)093
  [arXiv:1704.05340 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2018)093;%%
  %96 citations counted in INSPIRE as of 02 Feb 2018


%\cite{DescotesGenon:2012zf}
\bibitem{DescotesGenon:2012zf} 
  S.~Descotes-Genon, J.~Matias, M.~Ramon and J.~Virto,
  %``Implications from clean observables for the binned analysis of $B -> K*\mu^+\mu^-$ at large recoil,''
  JHEP {\bf 1301}, 048 (2013)
  doi:10.1007/JHEP01(2013)048
  [arXiv:1207.2753 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2013)048;%%
  %169 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hiller:2014ula}
\bibitem{Hiller:2014ula} 
  G.~Hiller and M.~Schmaltz,
  %``Diagnosing lepton-nonuniversality in $b \to s \ell \ell$,''
  JHEP {\bf 1502}, 055 (2015)
  doi:10.1007/JHEP02(2015)055
  [arXiv:1411.4773 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2015)055;%%
  %76 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Grygier:2017tzo}
\bibitem{Grygier:2017tzo} 
  J.~Grygier {\it et al.} [Belle Collaboration],
  %``Search for $\boldsymbol{B\to h\nu\bar{\nu}}$ decays with semileptonic tagging at Belle,''
  Phys.\ Rev.\ D {\bf 96}, no. 9, 091101 (2017)
  doi:10.1103/PhysRevD.96.091101
  [arXiv:1702.03224 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.96.091101;%%
  %22 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buras:2014fpa}
\bibitem{Buras:2014fpa} 
  A.~J.~Buras, J.~Girrbach-Noe, C.~Niehoff and D.~M.~Straub,
  %``$ B\to {K}^{\left(\ast \right)}\nu \overline{\nu} $ decays in the Standard Model and beyond,''
  JHEP {\bf 1502}, 184 (2015)
  doi:10.1007/JHEP02(2015)184
  [arXiv:1409.4557 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2015)184;%%
  %109 citations counted in INSPIRE as of 02 Feb 2018

%\cite{KouUrquijo}
  B2TiP Report (in progress).

%\cite{Dorsner:2016wpm}
\bibitem{Dorsner:2016wpm} 
  I.~Doršner, S.~Fajfer, A.~Greljo, J.~F.~Kamenik and N.~Košnik,
  %``Physics of leptoquarks in precision experiments and at particle colliders,''
  Phys.\ Rept.\  {\bf 641}, 1 (2016)
  doi:10.1016/j.physrep.2016.06.001
  [arXiv:1603.04993 [hep-ph]].
  %%CITATION = doi:10.1016/j.physrep.2016.06.001;%%
  %96 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Greljo:2015mma}
\bibitem{Greljo:2015mma} 
  A.~Greljo, G.~Isidori and D.~Marzocca,
  %``On the breaking of Lepton Flavor Universality in B decays,''
  JHEP {\bf 1507}, 142 (2015)
  doi:10.1007/JHEP07(2015)142
  [arXiv:1506.01705 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2015)142;%%
  %123 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Fajfer:2015ycq}
\bibitem{Fajfer:2015ycq} 
  S.~Fajfer and N.~Košnik,
  %``Vector leptoquark resolution of $R_K$ and $R_{D^{(*)}}$ puzzles,''
  Phys.\ Lett.\ B {\bf 755}, 270 (2016)
  doi:10.1016/j.physletb.2016.02.018
  [arXiv:1511.06024 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2016.02.018;%%
  %114 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Barbieri:2016las}
\bibitem{Barbieri:2016las} 
  R.~Barbieri, C.~W.~Murphy and F.~Senia,
  %``B-decay Anomalies in a Composite Leptoquark Model,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 1, 8 (2017)
  doi:10.1140/epjc/s10052-016-4578-7
  [arXiv:1611.04930 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-4578-7;%%
  %45 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Arnold:2012sd}
\bibitem{Arnold:2012sd} 
  J.~M.~Arnold, B.~Fornal and M.~B.~Wise,
  %``Simplified models with baryon number violation but no proton decay,''
  Phys.\ Rev.\ D {\bf 87}, 075004 (2013)
  doi:10.1103/PhysRevD.87.075004
  [arXiv:1212.4556 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.87.075004;%%
  %35 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Arnold:2013cva}
\bibitem{Arnold:2013cva} 
  J.~M.~Arnold, B.~Fornal and M.~B.~Wise,
  %``Phenomenology of scalar leptoquarks,''
  Phys.\ Rev.\ D {\bf 88}, 035009 (2013)
  doi:10.1103/PhysRevD.88.035009
  [arXiv:1304.6119 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.035009;%%
  %49 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Dorsner:2017wwn}
\bibitem{Dorsner:2017wwn} 
  I.~Doršner, S.~Fajfer and N.~Košnik,
  %``Leptoquark mechanism of neutrino masses within the grand unification framework,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 6, 417 (2017)
  doi:10.1140/epjc/s10052-017-4987-2
  [arXiv:1701.08322 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-4987-2;%%
  %7 citations counted in INSPIRE as of 02 Feb 2018


%\cite{1608.07583}
\bibitem{1608.07583} 
  D.~Bečirević, N.~Košnik, O.~Sumensari and R.~Zukanovich Funchal,
  %``Palatable Leptoquark Scenarios for Lepton Flavor Violation in Exclusive $b\to s\ell_1\ell_2$ modes,''
  JHEP {\bf 1611}, 035 (2016)
  doi:10.1007/JHEP11(2016)035
  [arXiv:1608.07583 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2016)035;%%
  %49 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Dorsner:2013tla}
\bibitem{Dorsner:2013tla} 
  I.~Doršner, S.~Fajfer, N.~Košnik and I.~Nišandžić,
  %``Minimally flavored colored scalar in $\bar B \to D^{(*)} \tau \bar \nu$ and the mass matrices constraints,''
  JHEP {\bf 1311}, 084 (2013)
  doi:10.1007/JHEP11(2013)084
  [arXiv:1306.6493 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2013)084;%%
  %85 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Freytsis:2015qca}
\bibitem{Freytsis:2015qca} 
  M.~Freytsis, Z.~Ligeti and J.~T.~Ruderman,
  %``Flavor models for $\bar{B} \to D^{(*)} \tau \bar{\nu}$,''
  Phys.\ Rev.\ D {\bf 92}, no. 5, 054018 (2015)
  doi:10.1103/PhysRevD.92.054018
  [arXiv:1506.08896 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.054018;%%
  %118 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Chauhan:2017ndd}
\bibitem{Chauhan:2017ndd} 
  B.~Chauhan, B.~Kindra and A.~Narang,
  %``A Leptoquark explanation for $(g-2)_\mu$, $R_K$, $R_{K^*}$ and, IceCube PeV events,''
  arXiv:1706.04598 [hep-ph].
  %%CITATION = ARXIV:1706.04598;%%
  %9 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Jegerlehner:2009ry}
\bibitem{Jegerlehner:2009ry} 
  F.~Jegerlehner and A.~Nyffeler,
  %``The Muon g-2,''
  Phys.\ Rept.\  {\bf 477}, 1 (2009)
  doi:10.1016/j.physrep.2009.04.003
  [arXiv:0902.3360 [hep-ph]].
  %%CITATION = doi:10.1016/j.physrep.2009.04.003;%%
  %733 citations counted in INSPIRE as of 02 Feb 2018


%\cite{NYFFELER:2014pta}
\bibitem{NYFFELER:2014pta} 
  A.~Nyffeler,
  %``Status of hadronic light-by-light scattering in the muon $g-2$,''
  Nuovo Cim.\ C {\bf 037}, no. 02, 173 (2014)
  [Int.\ J.\ Mod.\ Phys.\ Conf.\ Ser.\  {\bf 35}, 1460456 (2014)]
  doi:10.1393/ncc/i2014-11752-0, 10.1142/S2010194514604566
  [arXiv:1312.4804 [hep-ph]].
  %%CITATION = doi:10.1393/ncc/i2014-11752-0, 10.1142/S2010194514604566;%%
  %16 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Patrignani:2016xqp}
\bibitem{Patrignani:2016xqp} 
  C.~Patrignani {\it et al.} [Particle Data Group],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 40}, no. 10, 100001 (2016).
  doi:10.1088/1674-1137/40/10/100001
  %%CITATION = doi:10.1088/1674-1137/40/10/100001;%%
  %2536 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hazard:2016fnc}
\bibitem{Hazard:2016fnc} 
  D.~E.~Hazard and A.~A.~Petrov,
  %``Lepton flavor violating quarkonium decays,''
  Phys.\ Rev.\ D {\bf 94}, no. 7, 074023 (2016)
  doi:10.1103/PhysRevD.94.074023
  [arXiv:1607.00815 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.074023;%%
  %6 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Aloni:2017eny}
\bibitem{Aloni:2017eny} 
  D.~Aloni, A.~Efrati, Y.~Grossman and Y.~Nir,
  %``$\Upsilon$ and $\psi$ leptonic decays as probes of solutions to the $R_D^{(*)}$ puzzle,''
  JHEP {\bf 1706}, 019 (2017)
  doi:10.1007/JHEP06(2017)019
  [arXiv:1702.07356 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2017)019;%%
  %6 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Greljo:2017vvb}
\bibitem{Greljo:2017vvb} 
  A.~Greljo and D.~Marzocca,
  %``High-$p_T$ dilepton tails and flavor physics,''
  Eur.\ Phys.\ J.\ C {\bf 77}, no. 8, 548 (2017)
  doi:10.1140/epjc/s10052-017-5119-8
  [arXiv:1704.09015 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-5119-8;%%
  %27 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buchalla:1993wq}
\bibitem{Buchalla:1993wq} 
  G.~Buchalla and A.~J.~Buras,
  %``The rare decays $K^+ \to  \pi^+ \nu \bar \nu$ and $K_L \to  \mu^+ \mu^-$ beyond leading logarithms,''
  Nucl.\ Phys.\ B {\bf 412}, 106 (1994)
  doi:10.1016/0550-3213(94)90496-0
  [hep-ph/9308272].
  %%CITATION = doi:10.1016/0550-3213(94)90496-0;%%
  %248 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Misiak:1999yg}
\bibitem{Misiak:1999yg} 
  M.~Misiak and J.~Urban,
  %``QCD corrections to FCNC decays mediated by Z penguins and W boxes,''
  Phys.\ Lett.\ B {\bf 451}, 161 (1999)
  doi:10.1016/S0370-2693(99)00150-1
  [hep-ph/9901278].
  %%CITATION = doi:10.1016/S0370-2693(99)00150-1;%%
  %249 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Gorbahn:2004my}
\bibitem{Gorbahn:2004my} 
  M.~Gorbahn and U.~Haisch,
  %``Effective Hamiltonian for non-leptonic $|\Delta F| = 1$ decays at NNLO in QCD,''
  Nucl.\ Phys.\ B {\bf 713}, 291 (2005)
  doi:10.1016/j.nuclphysb.2005.01.047
  [hep-ph/0411071].
  %%CITATION = doi:10.1016/j.nuclphysb.2005.01.047;%%
  %176 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Isidori:2005xm}
\bibitem{Isidori:2005xm} 
  G.~Isidori, F.~Mescia and C.~Smith,
  %``Light-quark loops in K ---> pi nu anti-nu,''
  Nucl.\ Phys.\ B {\bf 718}, 319 (2005)
  doi:10.1016/j.nuclphysb.2005.04.008
  [hep-ph/0503107].
  %%CITATION = doi:10.1016/j.nuclphysb.2005.04.008;%%
  %153 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buras:2005gr}
\bibitem{Buras:2005gr} 
  A.~J.~Buras, M.~Gorbahn, U.~Haisch and U.~Nierste,
  %``The Rare decay K+ ---> pi+ nu anti-nu at the next-to-next-to-leading order in QCD,''
  Phys.\ Rev.\ Lett.\  {\bf 95}, 261805 (2005)
  doi:10.1103/PhysRevLett.95.261805
  [hep-ph/0508165].
  %%CITATION = doi:10.1103/PhysRevLett.95.261805;%%
  %146 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buras:2006gb}
\bibitem{Buras:2006gb} 
  A.~J.~Buras, M.~Gorbahn, U.~Haisch and U.~Nierste,
  %``Charm quark contribution to K+ ---> pi+ nu anti-nu at next-to-next-to-leading order,''
  JHEP {\bf 0611}, 002 (2006)
  Erratum: [JHEP {\bf 1211}, 167 (2012)]
  doi:10.1007/JHEP11(2012)167, 10.1088/1126-6708/2006/11/002
  [hep-ph/0603079].
  %%CITATION = doi:10.1007/JHEP11(2012)167, 10.1088/1126-6708/2006/11/002;%%
  %163 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Mescia:2007kn}
\bibitem{Mescia:2007kn} 
  F.~Mescia and C.~Smith,
  %``Improved estimates of rare K decay matrix-elements from Kl3 decays,''
  Phys.\ Rev.\ D {\bf 76}, 034017 (2007)
  doi:10.1103/PhysRevD.76.034017
  [arXiv:0705.2025 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.76.034017;%%
  %158 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Brod:2008ss}
\bibitem{Brod:2008ss} 
  J.~Brod and M.~Gorbahn,
  %``Electroweak Corrections to the Charm Quark Contribution to K+ ---> pi+ nu anti-nu,''
  Phys.\ Rev.\ D {\bf 78}, 034006 (2008)
  doi:10.1103/PhysRevD.78.034006
  [arXiv:0805.4119 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.78.034006;%%
  %126 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Brod:2010hi}
\bibitem{Brod:2010hi} 
  J.~Brod, M.~Gorbahn and E.~Stamou,
  %``Two-Loop Electroweak Corrections for the $K \to \pi \nu \bar{\nu}$ Decays,''
  Phys.\ Rev.\ D {\bf 83}, 034030 (2011)
  doi:10.1103/PhysRevD.83.034030
  [arXiv:1009.0947 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.83.034030;%%
  %230 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Buchalla:1998ba}
\bibitem{Buchalla:1998ba} 
  G.~Buchalla and A.~J.~Buras,
  %``The rare decays $K\to \pi \nu\bar\nu$, $B \to X \nu\bar\nu$ and $B \to l^+ l^-$: An Update,''
  Nucl.\ Phys.\ B {\bf 548}, 309 (1999)
  doi:10.1016/S0550-3213(99)00149-2
  [hep-ph/9901288].
  %%CITATION = doi:10.1016/S0550-3213(99)00149-2;%%
  %378 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Bai:2017fkh}
\bibitem{Bai:2017fkh} 
  Z.~Bai, N.~H.~Christ, X.~Feng, A.~Lawson, A.~Portelli and C.~T.~Sachrajda,
  %``Exploratory Lattice QCD Study of the Rare Kaon Decay $K^+\to\pi^+\nu\bar{\nu}$,''
  Phys.\ Rev.\ Lett.\  {\bf 118}, no. 25, 252001 (2017)
  doi:10.1103/PhysRevLett.118.252001
  [arXiv:1701.02858 [hep-lat]].
  %%CITATION = doi:10.1103/PhysRevLett.118.252001;%%
  %4 citations counted in INSPIRE as of 02 Feb 2018



\bibitem{JOcariz}
  CKMfitter Group, ``Prospective studies on $ K^+ \to \pi^+ \nu \nu $ and $ K_L \to \pi^0 \nu \nu $ rare kaon decays" (updated August 2015) at: http://ckmfitter.in2p3.fr
  

%\cite{Buras:2015qea}
\bibitem{Buras:2015qea} 
  A.~J.~Buras, D.~Buttazzo, J.~Girrbach-Noe and R.~Knegjens,
  %``$ {K}^{+}\to {\pi}^{+}\nu \overline{\nu} $ and $ {K}_L\to {\pi}^0\nu \overline{\nu} $ in the Standard Model: status and perspectives,''
  JHEP {\bf 1511}, 033 (2015)
  doi:10.1007/JHEP11(2015)033
  [arXiv:1503.02693 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2015)033;%%
  %120 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Adler:2001xv}
\bibitem{Adler:2001xv} 
  S.~Adler {\it et al.} [E787 Collaboration],
  %``Further evidence for the decay K+ ---> pi+ neutrino anti-neutrino,''
  Phys.\ Rev.\ Lett.\  {\bf 88}, 041803 (2002)
  doi:10.1103/PhysRevLett.88.041803
  [hep-ex/0111091].
  %%CITATION = doi:10.1103/PhysRevLett.88.041803;%%
  %193 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Anisimovsky:2004hr}
\bibitem{Anisimovsky:2004hr} 
  V.~V.~Anisimovsky {\it et al.} [E949 Collaboration],
  %``Improved measurement of the K+ ---> pi+ nu anti-nu branching ratio,''
  Phys.\ Rev.\ Lett.\  {\bf 93}, 031801 (2004)
  doi:10.1103/PhysRevLett.93.031801
  [hep-ex/0403036].
  %%CITATION = doi:10.1103/PhysRevLett.93.031801;%%
  %167 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Artamonov:2008qb}
\bibitem{Artamonov:2008qb} 
  A.~V.~Artamonov {\it et al.} [E949 Collaboration],
  %``New measurement of the $K^{+} \to \pi^{+} \nu \bar{\nu}$ branching ratio,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 191802 (2008)
  doi:10.1103/PhysRevLett.101.191802
  [arXiv:0808.2459 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.101.191802;%%
  %205 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Artamonov:2009sz}
\bibitem{Artamonov:2009sz} 
  A.~V.~Artamonov {\it et al.} [BNL-E949 Collaboration],
  %``Study of the decay $K^+\to\pi^+\nu \bar\nu$ in the momentum region $140 < P_\pi < 199$ MeV/c,''
  Phys.\ Rev.\ D {\bf 79}, 092004 (2009)
  doi:10.1103/PhysRevD.79.092004
  [arXiv:0903.0030 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.79.092004;%%
  %215 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Ahn:2009gb}
\bibitem{Ahn:2009gb} 
  J.~K.~Ahn {\it et al.} [E391a Collaboration],
  %``Experimental study of the decay K0(L) ---> pi0 nu nu-bar,''
  Phys.\ Rev.\ D {\bf 81}, 072004 (2010)
  doi:10.1103/PhysRevD.81.072004
  [arXiv:0911.4789 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.81.072004;%%
  %134 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Pepe:2015kaa}
\bibitem{Pepe:2015kaa} 
  M.~Pepe [NA62 Collaboration],
  %``Rare and forbidden kaon decays at NA62,''
  EPJ Web Conf.\  {\bf 95}, 03029 (2015).
  doi:10.1051/epjconf/20159503029, 10.1051/epjconf/20149503029
  %%CITATION = doi:10.1051/epjconf/20159503029, 10.1051/epjconf/20149503029;%%


%\cite{Shiomi:2014sfa}
\bibitem{Shiomi:2014sfa} 
  K.~Shiomi [KOTO Collaboration],
  %``$K^{0}_{L}\rightarrow \pi^{0} \nu \bar{\nu}$ at KOTO,''
  arXiv:1411.4250 [hep-ex].
  %%CITATION = ARXIV:1411.4250;%%
  %22 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Carpentier:2010ue}
\bibitem{Carpentier:2010ue} 
  M.~Carpentier and S.~Davidson,
  %``Constraints on two-lepton, two quark operators,''
  Eur.\ Phys.\ J.\ C {\bf 70}, 1071 (2010)
  doi:10.1140/epjc/s10052-010-1482-4
  [arXiv:1008.0280 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-010-1482-4;%%
  %62 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Isidori:2010kg}
\bibitem{Isidori:2010kg} 
  G.~Isidori, Y.~Nir and G.~Perez,
  %``Flavor Physics Constraints for Physics Beyond the Standard Model,''
  Ann.\ Rev.\ Nucl.\ Part.\ Sci.\  {\bf 60}, 355 (2010)
  doi:10.1146/annurev.nucl.012809.104534
  [arXiv:1002.0900 [hep-ph]].
  %%CITATION = doi:10.1146/annurev.nucl.012809.104534;%%
  %312 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Crivellin:2016vjc}
\bibitem{Crivellin:2016vjc} 
  A.~Crivellin, G.~D'Ambrosio, M.~Hoferichter and L.~C.~Tunstall,
  %``Violation of lepton flavor and lepton flavor universality in rare kaon decays,''
  Phys.\ Rev.\ D {\bf 93}, no. 7, 074038 (2016)
  doi:10.1103/PhysRevD.93.074038
  [arXiv:1601.00970 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.074038;%%
  %30 citations counted in INSPIRE as of 02 Feb 2018


\bibitem{CKMfitter} CKMfitter Group (J. Charles et al.), Eur. Phys. J. C41, 1-131 (2005) [hep-ph/0406184], updated results and plots available at: http://ckmfitter.in2p3.fr. The numerical values used here correspond to the results as of ICHEP 16. See references therein, and also references to the results as of Summer 15.


%\cite{Basecq:1985cr}
\bibitem{Basecq:1985cr} 
  J.~Basecq, L.~F.~Li and P.~B.~Pal,
  %``Gauge Invariant Calculation of the $K_L K_S$ Mass Difference in the Left-right Model,''
  Phys.\ Rev.\ D {\bf 32}, 175 (1985).
  doi:10.1103/PhysRevD.32.175
  %%CITATION = doi:10.1103/PhysRevD.32.175;%%
  %41 citations counted in INSPIRE as of 02 Feb 2018


%\cite{vanOldenborgh:1989wn}
\bibitem{vanOldenborgh:1989wn} 
  G.~J.~van Oldenborgh and J.~A.~M.~Vermaseren,
  %``New Algorithms for One Loop Integrals,''
  Z.\ Phys.\ C {\bf 46}, 425 (1990).
  doi:10.1007/BF01621031
  %%CITATION = doi:10.1007/BF01621031;%%
  %466 citations counted in INSPIRE as of 02 Feb 2018


%\cite{Hahn:1998yk}
\bibitem{Hahn:1998yk} 
  T.~Hahn and M.~Perez-Victoria,
  %``Automatized one loop calculations in four-dimensions and D-dimensions,''
  Comput.\ Phys.\ Commun.\  {\bf 118}, 153 (1999)
  doi:10.1016/S0010-4655(98)00173-8
  [hep-ph/9807565].
  %%CITATION = doi:10.1016/S0010-4655(98)00173-8;%%
  %1387 citations counted in INSPIRE as of 02 Feb 2018


%\cite{GagyiPalffy:1997hh}
\bibitem{GagyiPalffy:1997hh} 
  Z.~Gagyi-Palffy, A.~Pilaftsis and K.~Schilcher,
  %``Gauge independent analysis of K(L) ---> e mu in left-right models,''
  Nucl.\ Phys.\ B {\bf 513}, 517 (1998)
  doi:10.1016/S0550-3213(97)00764-5
  [hep-ph/9707517].
  %%CITATION = doi:10.1016/S0550-3213(97)00764-5;%%
  %25 citations counted in INSPIRE as of 02 Feb 2018

\end{thebibliography}
